A Reinforcement Learning Approach for Rebalancing Electric Vehicle Sharing Systems

This paper proposes a reinforcement learning approach for nightly offline rebalancing operations in free-floating electric vehicle sharing systems (FFEVSS). Due to sparse demand in a network, FFEVSS require relocation of electrical vehicles (EVs) to charging stations and demander nodes, which is typically done by a group of drivers. A shuttle is used to pick up and drop off drivers throughout the network. The objective of this study is to solve the shuttle routing problem to finish the rebalancing work in the minimal time. We consider a reinforcement learning framework for the problem, in which a central controller determines the routing policies of a fleet of multiple shuttles. We deploy a policy gradient method for training recurrent neural networks and compare the obtained policy results with heuristic solutions. Our numerical studies show that unlike the existing solutions in the literature, the proposed methods allow to solve the general version of the problem with no restrictions on the urban EV network structure and charging requirements of EVs. Moreover, the learned policies offer a wide range of flexibility resulting in a significant reduction in the time needed to rebalance the network.

==> bg.tex <==

\section{Background}



\subsection{Multi-agent Reinforcement Learning } 
Many important applications of reinforcement learning involve more than one agent (autonomous driving, robotics and etc.), which has given a rise to the development of multi-agent reinforcement learning. Similar to the single agent case, multi-agent reinforcement learning (MARL) solves sequential decision-making problems, where a set of autonomous agents share a common environment. Each agent aims to maximize it's own long-term return by interacting with environment and other agents. In \emph{fully cooperative} setting, all agents share a common long-term return . Fully collaborative setting also allows personal rewards for each agent that can be kept private, while the cooperation reward equals to the average rewards of all agents \cite{zhang2018fully}. 


There are some unique challenges of MARL that prohibit using the same theoretical frameworks as in single agent RL. For instance, stationary assumption of MDP is no longer valid in MARL setting. In particular, in the presence of other agents in environment the Markovian property, which states that reward and current state only depends on individual action and previous state,  does not hold. Indeed, individual rewards and state transitions depend on the actions of all agents, referred to as joint action. Another challenges of MARL involve multi-dimensional learning goals, which may include convergence to equilibrium points, efficiency of communication and others. Also, due to joint action space, where the combinations of all agents' actions need to be explored,  MARL suffers from scalability issues \cite{bucsoniu2010multi}.

\subsection{Decentralized Partially observable Markov Decision Processes}
A modeling framework commonly used in practice for multi-agent reinfocement learning is Decentralized Partially Observable Markov Decision Processes (Dec-POMDP). This framework consists of tuple ${\langle}\set{N}, \set{S}, \set{A}, P, R, \set{O}, O, \gamma {\rangle}$, where 
\begin{itemize}
	\item $\set{N} = \{1, ..., n\}$ is the set of $n$ agents
	\item $\set{S}$ is the set of global states
	\item $\set{A}$ is the set of joint actions such that $\set{A} = \set{A}^1 \times \set{A}^2 \times \cdots \times \set{A}^{n}$
	\item $P$ is the transition probability function 
	\item $R$ is the immediate reward function 
	\item $\set{O}$ is the set of joint observations such that $\set{O} = \set{O}^1 \times \set{O}^2 \times \cdots \times \set{O}^{n}$
	\item $O$ is the observation function 
	\item $\gamma$ is a discount factor.
\end{itemize}
At each time period $t$ each agent takes action $a^i_t$. Then joint action at period $t$ consists of actions of all agents $a_t = {\langle}a^1_t, a^1_t, \dots,  a^n_t  {\rangle}$. State transitions are governed by the transition probabilities function, which specifies $Pr(s_{t+1}|s_t, a_t)$. Agents do not observe state $s$, but indeed each agent $i$ has its local observation denoted by $o^i$. Similar to joint action, joint observation at time period $t$ is represented as $o_t = {\langle}o^1_t, o^1_t, \dots,  o^n_t  {\rangle}$. The observation function determines the probabilities of joint observations  $Pr(o_{t+1}|s_{t+1}, a_t)$. Reward function assigns the immediate reward $r_t$ given global state $s_t$ and joint action $a_t$. Then stochastic policy of each agents $i$ is based on its action-observation history denoted by $\tau^i:\set{O}^i\times \set{A}^i$ and can be represented as $\pi^i(a^i|\tau^i)$. 
A joint action-value function of joint policy can be written as $Q^{\pi}(s_t,a_t)=\mathbb{E}_{s_{t+1:T}, a_{t+1:T}}[R_t|s_t, a_t]$, where T is a planning horizon. $R_t = \sum_{k=0}^T\gamma^k r_{t+k}$ is the discounted return. 
Dec-POMDP modelling allows learning policies of agents in decentralized way \cite{oliehoek2016concise} and have been commonly used with the centralized training and decentralized execution paradigm \cite{rashid2020monotonic,son2019qtran, foerster2018counterfactual, lowe2017multi}.





\subsection{Actor-critic gradient methods in Multi-Agent Reinforcement Learning}
Similar to the single agent case, actor-critic methods have been adopted to multi-agent settings, where a critic estimates an action-value function according to which actor parameters are set to generate policies in the direction of improvement \cite{konda2000actor}. Actor-critic methods has been applied in various settings which allow a shared critic \cite{foerster2018counterfactual} and an individual critic per agent \cite{lowe2017multi, gupta2017cooperative}. For instance, \cite{foerster2018counterfactual} advocates a centralized training, where each agent has an actor network based only on local observations. All agents share a critic network, which is updated based on the global state. Then counterfactual advantage function is approximated to solve the credit assignment problem. Actor networks of each agent share parameters while the critic network is only used in the training phase. With the sufficient training actor networks produce decentralized policies. 
